Same Scene, Different Story: Evaluating Robot Perception Across Scene Phases in the Wild

Robots increasingly pick perception models off the shelf, and their errors propagate to the actions that follow. Yet these models are ranked task by task on separate leaderboards, not on the same scene as a robot changes it. We present \coolname{} (Robot Perception X): 100 real-world scenes captured with commodity RGB-D sensors before, during, and after manipulation, plus an egocentric view, with ground truth shared across six perception tasks. Two diagnostics, phase robustness~$\Phi$ and worst-phase quality~$\mathcal{J}_{\min}$, place every model on a common scale. Across 49 models and 65 zero-shot evaluations, the right model depends on the task and scene condition: depth and tracking show significant phase effects ($p{<}0.001$), rankings shift with prompting mode and input modality, and no evaluation reaches both $\mathcal{J}_{\min}{\geq}0.75$ and $\Phi{\geq}0.86$. \coolname{} pinpoints the phases and scene difficulty tiers where each model struggles; the dataset and toolkit are public. The project page is at https://irvlutd.github.io/RPX

==> generated/raw_t1_table.tex <==
\begin{table*}[tp]
\centering
\caption{T1 image depth: native metrics per phase. \textbf{Bold}: best; \underline{underlined}: each model's worst phase. Shade: per metric over all phases and models, lightest for the worst and darkest for the best value; \rpxHSwatchR\ higher, \rpxHSwatchL\ lower is better.}\label{tab:raw-t1}
\rpxHeatStyle{6.3}{2pt}
\begin{tabular}{@{}l@{\hspace{4.30pt}\hspace{5pt}\hspace{4.30pt}}ccc@{\hspace{4.30pt}\hspace{5pt}\hspace{4.30pt}}ccc@{\hspace{4.30pt}\hspace{5pt}\hspace{4.30pt}}ccc@{\hspace{4.30pt}\hspace{5pt}\hspace{4.30pt}}ccc@{}}
\rpxHTop
\rule{0pt}{9pt}\rpxHGroup{Model} & \multicolumn{3}{c}{\rpxHGroup{AbsRel\,\rpxDown{}}} & \multicolumn{3}{c}{\rpxHGroup{RMSE\,\rpxDown{}}} & \multicolumn{3}{c}{\rpxHGroup{SILog\,\rpxDown{}}} & \multicolumn{3}{c}{\rpxHGroup{$\delta_1$\,\rpxUp{}}} \\
\rpxHGroupRules{\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}}
& \rpxHHead{clu} & \rpxHHead{int} & \rpxHHead{cln} & \rpxHHead{clu} & \rpxHHead{int} & \rpxHHead{cln} & \rpxHHead{clu} & \rpxHHead{int} & \rpxHHead{cln} & \rpxHHead{clu} & \rpxHHead{int} & \rpxHHead{cln} \\
\rpxHMid
ZipDepth & \rpxHCell{rpxHL}{0.688}{\underline{0.167}} & \rpxHCell{rpxHL}{0.720}{0.161} & \rpxHCell{rpxHL}{0.736}{0.158} & \rpxHCell{rpxHL}{0.667}{0.454} & \rpxHCell{rpxHL}{0.534}{\underline{0.506}} & \rpxHCell{rpxHL}{0.593}{0.483} & \rpxHCell{rpxHL}{0.703}{15.51} & \rpxHCell{rpxHL}{0.544}{\underline{18.10}} & \rpxHCell{rpxHL}{0.718}{15.27} & \rpxHCell{rpxHR}{0.741}{\underline{0.732}} & \rpxHCell{rpxHR}{0.783}{0.761} & \rpxHCell{rpxHR}{0.776}{0.756} \\
HyDen & \rpxHCell{rpxHL}{0.150}{\underline{0.267}} & \rpxHCell{rpxHL}{0.252}{0.248} & \rpxHCell{rpxHL}{0.209}{0.256} & \rpxHCell{rpxHL}{0.231}{0.625} & \rpxHCell{rpxHL}{0.290}{0.602} & \rpxHCell{rpxHL}{0.150}{\underline{0.657}} & \rpxHCell{rpxHL}{0.903}{12.27} & \rpxHCell{rpxHL}{0.822}{\underline{13.58}} & \rpxHCell{rpxHL}{0.915}{12.07} & \rpxHCell{rpxHR}{0.150}{\underline{0.329}} & \rpxHCell{rpxHR}{0.201}{0.364} & \rpxHCell{rpxHR}{0.178}{0.348} \\
FE2E & \rpxHCell{rpxHL}{0.822}{0.142} & \rpxHCell{rpxHL}{0.833}{0.140} & \rpxHCell{rpxHL}{0.806}{\underline{0.145}} & \rpxHCell{rpxHL}{0.850}{0.382} & \rpxHCell{rpxHL}{0.684}{\underline{0.447}} & \rpxHCell{rpxHL}{0.705}{0.439} & \rpxHCell{rpxHL}{0.934}{11.77} & \rpxHCell{rpxHL}{0.757}{\underline{14.63}} & \rpxHCell{rpxHL}{0.887}{12.53} & \rpxHCell{rpxHR}{0.862}{0.815} & \rpxHCell{rpxHR}{0.889}{0.833} & \rpxHCell{rpxHR}{0.851}{\underline{0.807}} \\
DA3 Metric-L & \rpxHCell{rpxHL}{0.909}{\underline{0.126}} & \rpxHCell{rpxHL}{0.957}{0.117} & \rpxHCell{rpxHL}{0.952}{\textbf{0.118}} & \rpxHCell{rpxHL}{1.000}{\textbf{0.323}} & \rpxHCell{rpxHL}{0.837}{\underline{0.387}} & \rpxHCell{rpxHL}{0.901}{\textbf{0.362}} & \rpxHCell{rpxHL}{0.999}{\textbf{10.71}} & \rpxHCell{rpxHL}{0.817}{\underline{13.67}} & \rpxHCell{rpxHL}{0.978}{11.05} & \rpxHCell{rpxHR}{0.912}{\underline{\textbf{0.849}}} & \rpxHCell{rpxHR}{1.000}{\textbf{0.909}} & \rpxHCell{rpxHR}{0.943}{\textbf{0.870}} \\
UniDepth V2 & \rpxHCell{rpxHL}{0.822}{\underline{0.142}} & \rpxHCell{rpxHL}{0.909}{0.126} & \rpxHCell{rpxHL}{0.892}{0.129} & \rpxHCell{rpxHL}{0.921}{0.354} & \rpxHCell{rpxHL}{0.822}{\underline{0.393}} & \rpxHCell{rpxHL}{0.837}{0.387} & \rpxHCell{rpxHL}{0.977}{11.07} & \rpxHCell{rpxHL}{0.831}{\underline{13.44}} & \rpxHCell{rpxHL}{1.000}{\textbf{10.69}} & \rpxHCell{rpxHR}{0.840}{\underline{0.800}} & \rpxHCell{rpxHR}{0.965}{0.885} & \rpxHCell{rpxHR}{0.884}{0.830} \\
MoGe-2 ViT-L & \rpxHCell{rpxHL}{0.225}{\underline{0.253}} & \rpxHCell{rpxHL}{0.451}{0.211} & \rpxHCell{rpxHL}{0.365}{0.227} & \rpxHCell{rpxHL}{0.450}{0.539} & \rpxHCell{rpxHL}{0.509}{0.516} & \rpxHCell{rpxHL}{0.415}{\underline{0.553}} & \rpxHCell{rpxHL}{0.970}{11.18} & \rpxHCell{rpxHL}{0.825}{\underline{13.53}} & \rpxHCell{rpxHL}{0.958}{11.37} & \rpxHCell{rpxHR}{0.225}{\underline{0.380}} & \rpxHCell{rpxHR}{0.462}{0.542} & \rpxHCell{rpxHR}{0.370}{0.479} \\
Lotus-2 & \rpxHCell{rpxHL}{0.397}{\underline{0.221}} & \rpxHCell{rpxHL}{0.505}{0.201} & \rpxHCell{rpxHL}{0.414}{0.218} & \rpxHCell{rpxHL}{0.677}{0.450} & \rpxHCell{rpxHL}{0.570}{\underline{0.492}} & \rpxHCell{rpxHL}{0.572}{0.491} & \rpxHCell{rpxHL}{0.192}{23.82} & \rpxHCell{rpxHL}{0.263}{22.67} & \rpxHCell{rpxHL}{0.150}{\underline{24.50}} & \rpxHCell{rpxHR}{0.591}{\underline{0.630}} & \rpxHCell{rpxHR}{0.659}{0.676} & \rpxHCell{rpxHR}{0.600}{0.636} \\
Depth Pro & \rpxHCell{rpxHL}{0.672}{\underline{0.170}} & \rpxHCell{rpxHL}{0.839}{0.139} & \rpxHCell{rpxHL}{0.699}{0.165} & \rpxHCell{rpxHL}{0.687}{0.446} & \rpxHCell{rpxHL}{0.651}{0.460} & \rpxHCell{rpxHL}{0.570}{\underline{0.492}} & \rpxHCell{rpxHL}{0.859}{12.98} & \rpxHCell{rpxHL}{0.743}{\underline{14.86}} & \rpxHCell{rpxHL}{0.866}{12.86} & \rpxHCell{rpxHR}{0.710}{\underline{0.711}} & \rpxHCell{rpxHR}{0.925}{0.858} & \rpxHCell{rpxHR}{0.746}{0.736} \\
Metric3D V2 & \rpxHCell{rpxHL}{0.919}{\underline{\textbf{0.124}}} & \rpxHCell{rpxHL}{1.000}{\textbf{0.109}} & \rpxHCell{rpxHL}{0.925}{0.123} & \rpxHCell{rpxHL}{0.903}{0.361} & \rpxHCell{rpxHL}{0.845}{\textbf{0.384}} & \rpxHCell{rpxHL}{0.789}{\underline{0.406}} & \rpxHCell{rpxHL}{0.956}{11.41} & \rpxHCell{rpxHL}{0.861}{\underline{\textbf{12.95}}} & \rpxHCell{rpxHL}{0.957}{11.39} & \rpxHCell{rpxHR}{0.906}{0.845} & \rpxHCell{rpxHR}{0.999}{0.908} & \rpxHCell{rpxHR}{0.894}{\underline{0.837}} \\
DA-V2 Large & \rpxHCell{rpxHL}{0.457}{0.210} & \rpxHCell{rpxHL}{0.424}{\underline{0.216}} & \rpxHCell{rpxHL}{0.736}{0.158} & \rpxHCell{rpxHL}{0.824}{0.392} & \rpxHCell{rpxHL}{0.524}{\underline{0.510}} & \rpxHCell{rpxHL}{0.829}{0.390} & \rpxHCell{rpxHL}{0.886}{12.54} & \rpxHCell{rpxHL}{0.713}{\underline{15.35}} & \rpxHCell{rpxHL}{0.867}{12.85} & \rpxHCell{rpxHR}{0.700}{0.704} & \rpxHCell{rpxHR}{0.688}{\underline{0.696}} & \rpxHCell{rpxHR}{0.846}{0.804} \\
\rpxHMid
\textcolor{rpxHMute}{\textit{Times worst}} & \textcolor{rpxHMute}{8} & \textcolor{rpxHMute}{1} & \textcolor{rpxHMute}{1} & \textcolor{rpxHMute}{0} & \textcolor{rpxHMute}{6} & \textcolor{rpxHMute}{4} & \textcolor{rpxHMute}{0} & \textcolor{rpxHMute}{9} & \textcolor{rpxHMute}{1} & \textcolor{rpxHMute}{7} & \textcolor{rpxHMute}{1} & \textcolor{rpxHMute}{2} \\
\rpxHBottom
\end{tabular}
\end{table*}


==> generated/raw_t3_table.tex <==
\begin{table*}[tp]
\centering
\begin{minipage}[t]{0.60\textwidth}\centering
\caption{T3 multi-object tracking: native metrics per view and phase. \textbf{Bold}: best; \underline{underlined}: each model's worst phase or view. Shade: \rpxHSwatchR\ higher and \rpxHSwatchL\ lower is better, as in Table~\ref{tab:raw-t1}.}\label{tab:raw-t3}
\rpxHeatStyle{5.7}{2pt}\setlength{\tabcolsep}{1.35pt}
\begin{tabular}{@{}l@{\hspace{1.80pt}\hspace{5pt}\hspace{1.80pt}}cccc@{\hspace{1.80pt}\hspace{5pt}\hspace{1.80pt}}cccc@{\hspace{1.80pt}\hspace{5pt}\hspace{1.80pt}}cccc@{}}
\rpxHTop
\rule{0pt}{9pt}\rpxHGroup{Model} & \multicolumn{4}{c}{\rpxHGroup{HOTA\,\rpxUp{}}} & \multicolumn{4}{c}{\rpxHGroup{MOTA\,\rpxUp{}}} & \multicolumn{4}{c}{\rpxHGroup{IDSW\,\rpxDown{}}} \\
\rpxHGroupRules{\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}}
& \rpxHHead{clu} & \rpxHHead{int} & \rpxHHead{cln} & \rpxHHead{ego} & \rpxHHead{clu} & \rpxHHead{int} & \rpxHHead{cln} & \rpxHHead{ego} & \rpxHHead{clu} & \rpxHHead{int} & \rpxHHead{cln} & \rpxHHead{ego} \\
\rpxHMid
SAM 2 Long & \rpxHCell{rpxHR}{0.994}{\textbf{0.973}} & \rpxHCell{rpxHR}{0.867}{\underline{\textbf{0.930}}} & \rpxHCell{rpxHR}{1.000}{\textbf{0.975}} & \rpxHCell{rpxHR}{0.932}{\textbf{0.952}} & \rpxHCell{rpxHR}{0.983}{\textbf{0.983}} & \rpxHCell{rpxHR}{0.888}{\underline{\textbf{0.938}}} & \rpxHCell{rpxHR}{1.000}{\textbf{0.991}} & \rpxHCell{rpxHR}{0.919}{\textbf{0.953}} & \rpxHCell{rpxHL}{0.900}{0.65} & \rpxHCell{rpxHL}{0.803}{1.10} & \rpxHCell{rpxHL}{0.996}{0.21} & \rpxHCell{rpxHL}{0.666}{\underline{1.73}} \\
DAM4SAM & \rpxHCell{rpxHR}{0.979}{0.968} & \rpxHCell{rpxHR}{0.846}{\underline{0.923}} & \rpxHCell{rpxHR}{0.997}{0.974} & \rpxHCell{rpxHR}{0.902}{0.942} & \rpxHCell{rpxHR}{0.962}{0.973} & \rpxHCell{rpxHR}{0.854}{\underline{0.922}} & \rpxHCell{rpxHR}{0.992}{0.987} & \rpxHCell{rpxHR}{0.888}{0.938} & \rpxHCell{rpxHL}{0.874}{0.77} & \rpxHCell{rpxHL}{0.623}{1.93} & \rpxHCell{rpxHL}{0.996}{0.21} & \rpxHCell{rpxHL}{0.456}{\underline{2.70}} \\
EdgeTAM & \rpxHCell{rpxHR}{0.923}{0.949} & \rpxHCell{rpxHR}{0.742}{0.888} & \rpxHCell{rpxHR}{0.941}{0.955} & \rpxHCell{rpxHR}{0.730}{\underline{0.884}} & \rpxHCell{rpxHR}{0.949}{0.967} & \rpxHCell{rpxHR}{0.784}{0.889} & \rpxHCell{rpxHR}{0.975}{0.979} & \rpxHCell{rpxHR}{0.758}{\underline{0.877}} & \rpxHCell{rpxHL}{0.909}{0.61} & \rpxHCell{rpxHL}{0.774}{1.23} & \rpxHCell{rpxHL}{0.991}{0.23} & \rpxHCell{rpxHL}{0.642}{\underline{1.84}} \\
SAM 2++ & \rpxHCell{rpxHR}{0.938}{0.954} & \rpxHCell{rpxHR}{0.748}{0.890} & \rpxHCell{rpxHR}{0.947}{0.957} & \rpxHCell{rpxHR}{0.520}{\underline{0.813}} & \rpxHCell{rpxHR}{0.962}{0.973} & \rpxHCell{rpxHR}{0.767}{0.881} & \rpxHCell{rpxHR}{0.975}{0.979} & \rpxHCell{rpxHR}{0.563}{\underline{0.785}} & \rpxHCell{rpxHL}{0.950}{0.42} & \rpxHCell{rpxHL}{0.783}{\underline{1.19}} & \rpxHCell{rpxHL}{0.989}{0.24} & \rpxHCell{rpxHL}{0.879}{\textbf{0.75}} \\
SAM 2 & \rpxHCell{rpxHR}{0.976}{0.967} & \rpxHCell{rpxHR}{0.840}{0.921} & \rpxHCell{rpxHR}{0.985}{0.970} & \rpxHCell{rpxHR}{0.790}{\underline{0.904}} & \rpxHCell{rpxHR}{0.970}{0.977} & \rpxHCell{rpxHR}{0.856}{0.923} & \rpxHCell{rpxHR}{0.987}{0.985} & \rpxHCell{rpxHR}{0.782}{\underline{0.888}} & \rpxHCell{rpxHL}{0.911}{0.60} & \rpxHCell{rpxHL}{0.764}{1.28} & \rpxHCell{rpxHL}{0.996}{0.21} & \rpxHCell{rpxHL}{0.608}{\underline{2.00}} \\
Cutie & \rpxHCell{rpxHR}{0.908}{0.944} & \rpxHCell{rpxHR}{0.751}{\underline{0.891}} & \rpxHCell{rpxHR}{0.941}{0.955} & \rpxHCell{rpxHR}{0.790}{0.904} & \rpxHCell{rpxHR}{0.953}{0.969} & \rpxHCell{rpxHR}{0.820}{\underline{0.906}} & \rpxHCell{rpxHR}{0.994}{0.988} & \rpxHCell{rpxHR}{0.830}{0.911} & \rpxHCell{rpxHL}{0.915}{0.58} & \rpxHCell{rpxHL}{0.801}{1.11} & \rpxHCell{rpxHL}{1.000}{\textbf{0.19}} & \rpxHCell{rpxHL}{0.707}{\underline{1.54}} \\
SAM 3.1 (bbox) & \rpxHCell{rpxHR}{0.944}{0.956} & \rpxHCell{rpxHR}{0.594}{\underline{0.838}} & \rpxHCell{rpxHR}{0.935}{0.953} & \rpxHCell{rpxHR}{0.736}{0.886} & \rpxHCell{rpxHR}{0.958}{0.971} & \rpxHCell{rpxHR}{0.629}{\underline{0.816}} & \rpxHCell{rpxHR}{0.962}{0.973} & \rpxHCell{rpxHR}{0.754}{0.875} & \rpxHCell{rpxHL}{0.907}{0.62} & \rpxHCell{rpxHL}{0.690}{1.62} & \rpxHCell{rpxHL}{0.974}{0.31} & \rpxHCell{rpxHL}{0.616}{\underline{1.96}} \\
MiTS & \rpxHCell{rpxHR}{0.805}{0.909} & \rpxHCell{rpxHR}{0.544}{\underline{0.821}} & \rpxHCell{rpxHR}{0.870}{0.931} & \rpxHCell{rpxHR}{0.562}{0.827} & \rpxHCell{rpxHR}{0.894}{0.941} & \rpxHCell{rpxHR}{0.599}{0.802} & \rpxHCell{rpxHR}{0.932}{0.959} & \rpxHCell{rpxHR}{0.563}{\underline{0.785}} & \rpxHCell{rpxHL}{0.907}{0.62} & \rpxHCell{rpxHL}{0.575}{2.15} & \rpxHCell{rpxHL}{1.000}{\textbf{0.19}} & \rpxHCell{rpxHL}{0.232}{\underline{3.73}} \\
XMem & \rpxHCell{rpxHR}{0.858}{0.927} & \rpxHCell{rpxHR}{0.615}{\underline{0.845}} & \rpxHCell{rpxHR}{0.911}{0.945} & \rpxHCell{rpxHR}{0.683}{0.868} & \rpxHCell{rpxHR}{0.930}{0.958} & \rpxHCell{rpxHR}{0.654}{\underline{0.828}} & \rpxHCell{rpxHR}{0.972}{0.978} & \rpxHCell{rpxHR}{0.724}{0.861} & \rpxHCell{rpxHL}{0.970}{\textbf{0.33}} & \rpxHCell{rpxHL}{0.766}{1.27} & \rpxHCell{rpxHL}{1.000}{\textbf{0.19}} & \rpxHCell{rpxHL}{0.718}{\underline{1.49}} \\
SAM 3.1 (text) & \rpxHCell{rpxHR}{0.523}{0.814} & \rpxHCell{rpxHR}{0.150}{\underline{0.688}} & \rpxHCell{rpxHR}{0.491}{0.803} & \rpxHCell{rpxHR}{0.310}{0.742} & \rpxHCell{rpxHR}{0.470}{0.741} & \rpxHCell{rpxHR}{0.150}{\underline{0.590}} & \rpxHCell{rpxHR}{0.449}{0.731} & \rpxHCell{rpxHR}{0.332}{0.676} & \rpxHCell{rpxHL}{0.868}{0.80} & \rpxHCell{rpxHL}{0.657}{1.77} & \rpxHCell{rpxHL}{0.840}{0.93} & \rpxHCell{rpxHL}{0.150}{\underline{4.11}} \\
GSAM2 (text) & \rpxHCell{rpxHR}{0.674}{0.865} & \rpxHCell{rpxHR}{0.411}{\underline{0.776}} & \rpxHCell{rpxHR}{0.730}{0.884} & \rpxHCell{rpxHR}{0.609}{0.843} & \rpxHCell{rpxHR}{0.546}{0.777} & \rpxHCell{rpxHR}{0.262}{\underline{0.643}} & \rpxHCell{rpxHR}{0.635}{0.819} & \rpxHCell{rpxHR}{0.504}{0.757} & \rpxHCell{rpxHL}{0.928}{0.52} & \rpxHCell{rpxHL}{0.905}{\textbf{0.63}} & \rpxHCell{rpxHL}{0.993}{0.22} & \rpxHCell{rpxHL}{0.716}{\underline{1.50}} \\
\rpxHMid
\textcolor{rpxHMute}{\textit{Times worst}} & \textcolor{rpxHMute}{0} & \textcolor{rpxHMute}{8} & \textcolor{rpxHMute}{0} & \textcolor{rpxHMute}{3} & \textcolor{rpxHMute}{0} & \textcolor{rpxHMute}{7} & \textcolor{rpxHMute}{0} & \textcolor{rpxHMute}{4} & \textcolor{rpxHMute}{0} & \textcolor{rpxHMute}{1} & \textcolor{rpxHMute}{0} & \textcolor{rpxHMute}{10} \\
\rpxHBottom
\end{tabular}
\end{minipage}\hfill
\begin{minipage}[t]{0.38\textwidth}\centering
\caption{T4 relative camera pose: native metrics for the Clutter and Clean pair sets. \textbf{Bold}: best; \underline{underlined}: each model's worst pair set. Shade: \rpxHSwatchR\ higher and \rpxHSwatchL\ lower is better, as in Table~\ref{tab:raw-t1}.}\label{tab:raw-t4}
\rpxHeatStyle{5.7}{2pt}\setlength{\tabcolsep}{0.9pt}
\begin{tabular}{@{}l@{\hspace{1.30pt}\hspace{5pt}\hspace{1.30pt}}cc@{\hspace{1.30pt}\hspace{5pt}\hspace{1.30pt}}cc@{\hspace{1.30pt}\hspace{5pt}\hspace{1.30pt}}cc@{}}
\rpxHTop
\rule{0pt}{9pt}\rpxHGroup{Model} & \multicolumn{2}{c}{\rpxHGroup{AUC@5$^\circ$\,\rpxUp{}}} & \multicolumn{2}{c}{\rpxHGroup{AUC@10$^\circ$\,\rpxUp{}}} & \multicolumn{2}{c}{\rpxHGroup{AUC@20$^\circ$\,\rpxUp{}}} \\
\rpxHGroupRules{\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}}
& \rpxHHead{clu} & \rpxHHead{cln} & \rpxHHead{clu} & \rpxHHead{cln} & \rpxHHead{clu} & \rpxHHead{cln} \\
\rpxHMid
DA3 & \rpxHCell{rpxHR}{0.787}{\underline{\textbf{0.205}}} & \rpxHCell{rpxHR}{1.000}{\textbf{0.263}} & \rpxHCell{rpxHR}{0.872}{\underline{\textbf{0.454}}} & \rpxHCell{rpxHR}{1.000}{\textbf{0.518}} & \rpxHCell{rpxHR}{0.926}{\underline{\textbf{0.685}}} & \rpxHCell{rpxHR}{1.000}{\textbf{0.729}} \\
VGGT & \rpxHCell{rpxHR}{0.678}{\underline{0.175}} & \rpxHCell{rpxHR}{0.857}{0.224} & \rpxHCell{rpxHR}{0.773}{\underline{0.404}} & \rpxHCell{rpxHR}{0.910}{0.473} & \rpxHCell{rpxHR}{0.844}{\underline{0.636}} & \rpxHCell{rpxHR}{0.941}{0.694} \\
Reloc3R & \rpxHCell{rpxHR}{0.762}{\underline{0.198}} & \rpxHCell{rpxHR}{0.923}{0.242} & \rpxHCell{rpxHR}{0.848}{\underline{0.442}} & \rpxHCell{rpxHR}{0.954}{0.495} & \rpxHCell{rpxHR}{0.904}{\underline{0.672}} & \rpxHCell{rpxHR}{0.968}{0.710} \\
Pi3X & \rpxHCell{rpxHR}{0.700}{\underline{0.181}} & \rpxHCell{rpxHR}{0.872}{0.228} & \rpxHCell{rpxHR}{0.787}{\underline{0.411}} & \rpxHCell{rpxHR}{0.916}{0.476} & \rpxHCell{rpxHR}{0.859}{\underline{0.645}} & \rpxHCell{rpxHR}{0.945}{0.696} \\
MonST3R & \rpxHCell{rpxHR}{0.150}{\underline{0.031}} & \rpxHCell{rpxHR}{0.201}{0.045} & \rpxHCell{rpxHR}{0.150}{\underline{0.092}} & \rpxHCell{rpxHR}{0.226}{0.130} & \rpxHCell{rpxHR}{0.150}{\underline{0.222}} & \rpxHCell{rpxHR}{0.264}{0.290} \\
MUSt3R & \rpxHCell{rpxHR}{0.436}{\underline{0.109}} & \rpxHCell{rpxHR}{0.560}{0.143} & \rpxHCell{rpxHR}{0.559}{\underline{0.297}} & \rpxHCell{rpxHR}{0.659}{0.347} & \rpxHCell{rpxHR}{0.676}{\underline{0.536}} & \rpxHCell{rpxHR}{0.760}{0.586} \\
Fast3R & \rpxHCell{rpxHR}{0.458}{\underline{0.115}} & \rpxHCell{rpxHR}{0.535}{0.136} & \rpxHCell{rpxHR}{0.601}{\underline{0.318}} & \rpxHCell{rpxHR}{0.669}{0.352} & \rpxHCell{rpxHR}{0.740}{\underline{0.574}} & \rpxHCell{rpxHR}{0.782}{0.599} \\
CUT3R & \rpxHCell{rpxHR}{0.494}{\underline{0.125}} & \rpxHCell{rpxHR}{0.652}{0.168} & \rpxHCell{rpxHR}{0.633}{\underline{0.334}} & \rpxHCell{rpxHR}{0.759}{0.397} & \rpxHCell{rpxHR}{0.754}{\underline{0.582}} & \rpxHCell{rpxHR}{0.839}{0.633} \\
MASt3R & \rpxHCell{rpxHR}{0.641}{\underline{0.165}} & \rpxHCell{rpxHR}{0.777}{0.202} & \rpxHCell{rpxHR}{0.719}{\underline{0.377}} & \rpxHCell{rpxHR}{0.826}{0.431} & \rpxHCell{rpxHR}{0.774}{\underline{0.594}} & \rpxHCell{rpxHR}{0.861}{0.646} \\
DUSt3R & \rpxHCell{rpxHR}{0.286}{\underline{0.068}} & \rpxHCell{rpxHR}{0.326}{0.079} & \rpxHCell{rpxHR}{0.365}{\underline{0.200}} & \rpxHCell{rpxHR}{0.409}{0.222} & \rpxHCell{rpxHR}{0.465}{\underline{0.410}} & \rpxHCell{rpxHR}{0.512}{0.438} \\
\rpxHMid
\textcolor{rpxHMute}{\textit{Times worst}} & \textcolor{rpxHMute}{10} & \textcolor{rpxHMute}{0} & \textcolor{rpxHMute}{10} & \textcolor{rpxHMute}{0} & \textcolor{rpxHMute}{10} & \textcolor{rpxHMute}{0} \\
\rpxHBottom
\end{tabular}
\end{minipage}
\end{table*}


==> generated/raw_t5_table.tex <==
\begin{table*}[tp]
\centering
\caption{T5 regular VQA: native grounding metrics per view and phase (Center: Center-in-GT), pooled over all eight planned question types, including the unscored spatial types, so they are not the inputs of the published $\mathcal J$, which uses the five attribute types. \textbf{Bold}: best; \underline{underlined}: each model's worst phase or view. Shade: \rpxHSwatchR\ higher and \rpxHSwatchL\ lower is better, as in Table~\ref{tab:raw-t1}.}\label{tab:raw-t5}
\rpxHeatStyle{6.3}{2pt}
\begin{rpxfit}{\textwidth}{18}{@{}l@{}@{\hspace{3.30pt}\hspace{5pt}\hspace{3.30pt}}cccc@{\hspace{3.30pt}\hspace{5pt}\hspace{3.30pt}}cccc@{\hspace{3.30pt}\hspace{5pt}\hspace{3.30pt}}cccc@{}}
\rpxHTop
\rule{0pt}{9pt}\rpxHGroup{Model} & \multicolumn{4}{c}{\rpxHGroup{Acc@0.5\,\rpxUp{}}} & \multicolumn{4}{c}{\rpxHGroup{GIoU\,\rpxUp{}}} & \multicolumn{4}{c}{\rpxHGroup{Center\,\rpxUp{}}} \\
\rpxHGroupRules{\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}}
& \rpxHHead{clu} & \rpxHHead{int} & \rpxHHead{cln} & \rpxHHead{ego} & \rpxHHead{clu} & \rpxHHead{int} & \rpxHHead{cln} & \rpxHHead{ego} & \rpxHHead{clu} & \rpxHHead{int} & \rpxHHead{cln} & \rpxHHead{ego} \\
\rpxHMid
Cosmos Reason2 8B & \rpxHCell{rpxHR}{0.761}{\textbf{0.489}} & \rpxHCell{rpxHR}{0.671}{\underline{\textbf{0.425}}} & \rpxHCell{rpxHR}{0.757}{\textbf{0.486}} & \rpxHCell{rpxHR}{0.962}{0.632} & \rpxHCell{rpxHR}{0.777}{0.188} & \rpxHCell{rpxHR}{0.682}{\underline{0.077}} & \rpxHCell{rpxHR}{0.713}{0.113} & \rpxHCell{rpxHR}{0.971}{0.416} & \rpxHCell{rpxHR}{0.781}{\textbf{0.541}} & \rpxHCell{rpxHR}{0.680}{\underline{\textbf{0.476}}} & \rpxHCell{rpxHR}{0.742}{\textbf{0.516}} & \rpxHCell{rpxHR}{0.973}{0.664} \\
Cosmos Reason2 2B & \rpxHCell{rpxHR}{0.359}{0.203} & \rpxHCell{rpxHR}{0.317}{0.173} & \rpxHCell{rpxHR}{0.316}{\underline{0.172}} & \rpxHCell{rpxHR}{0.574}{0.356} & \rpxHCell{rpxHR}{0.281}{$-$0.393} & \rpxHCell{rpxHR}{0.187}{$-$0.504} & \rpxHCell{rpxHR}{0.150}{\underline{$-$0.547}} & \rpxHCell{rpxHR}{0.462}{$-$0.181} & \rpxHCell{rpxHR}{0.333}{0.254} & \rpxHCell{rpxHR}{0.266}{0.211} & \rpxHCell{rpxHR}{0.244}{\underline{0.197}} & \rpxHCell{rpxHR}{0.542}{0.388} \\
Qwen3-VL 8B & \rpxHCell{rpxHR}{0.749}{0.480} & \rpxHCell{rpxHR}{0.612}{\underline{0.383}} & \rpxHCell{rpxHR}{0.744}{0.477} & \rpxHCell{rpxHR}{1.000}{\textbf{0.659}} & \rpxHCell{rpxHR}{0.849}{\textbf{0.273}} & \rpxHCell{rpxHR}{0.704}{\underline{\textbf{0.103}}} & \rpxHCell{rpxHR}{0.759}{\textbf{0.167}} & \rpxHCell{rpxHR}{1.000}{\textbf{0.450}} & \rpxHCell{rpxHR}{0.755}{0.524} & \rpxHCell{rpxHR}{0.597}{\underline{0.423}} & \rpxHCell{rpxHR}{0.716}{0.499} & \rpxHCell{rpxHR}{1.000}{\textbf{0.681}} \\
Qwen3-VL 2B & \rpxHCell{rpxHR}{0.491}{0.297} & \rpxHCell{rpxHR}{0.479}{\underline{0.288}} & \rpxHCell{rpxHR}{0.507}{0.308} & \rpxHCell{rpxHR}{0.909}{0.594} & \rpxHCell{rpxHR}{0.457}{$-$0.187} & \rpxHCell{rpxHR}{0.425}{$-$0.225} & \rpxHCell{rpxHR}{0.404}{\underline{$-$0.249}} & \rpxHCell{rpxHR}{0.885}{0.315} & \rpxHCell{rpxHR}{0.433}{0.318} & \rpxHCell{rpxHR}{0.411}{\underline{0.304}} & \rpxHCell{rpxHR}{0.433}{0.318} & \rpxHCell{rpxHR}{0.887}{0.609} \\
InternVL 3.5 14B & \rpxHCell{rpxHR}{0.664}{0.420} & \rpxHCell{rpxHR}{0.505}{\underline{0.307}} & \rpxHCell{rpxHR}{0.621}{0.389} & \rpxHCell{rpxHR}{0.779}{0.502} & \rpxHCell{rpxHR}{0.831}{0.252} & \rpxHCell{rpxHR}{0.675}{\underline{0.069}} & \rpxHCell{rpxHR}{0.744}{0.150} & \rpxHCell{rpxHR}{0.831}{0.252} & \rpxHCell{rpxHR}{0.653}{0.459} & \rpxHCell{rpxHR}{0.481}{\underline{0.349}} & \rpxHCell{rpxHR}{0.598}{0.424} & \rpxHCell{rpxHR}{0.766}{0.531} \\
InternVL 3.5 1B & \rpxHCell{rpxHR}{0.583}{0.362} & \rpxHCell{rpxHR}{0.490}{\underline{0.296}} & \rpxHCell{rpxHR}{0.576}{0.357} & \rpxHCell{rpxHR}{0.522}{0.319} & \rpxHCell{rpxHR}{0.743}{0.149} & \rpxHCell{rpxHR}{0.625}{\underline{0.010}} & \rpxHCell{rpxHR}{0.651}{0.041} & \rpxHCell{rpxHR}{0.626}{0.011} & \rpxHCell{rpxHR}{0.612}{0.433} & \rpxHCell{rpxHR}{0.511}{\underline{0.368}} & \rpxHCell{rpxHR}{0.569}{0.405} & \rpxHCell{rpxHR}{0.606}{0.429} \\
PaliGemma 2 10B & \rpxHCell{rpxHR}{0.573}{0.355} & \rpxHCell{rpxHR}{0.460}{\underline{0.275}} & \rpxHCell{rpxHR}{0.524}{0.320} & \rpxHCell{rpxHR}{0.604}{0.377} & \rpxHCell{rpxHR}{0.674}{0.068} & \rpxHCell{rpxHR}{0.511}{\underline{$-$0.124}} & \rpxHCell{rpxHR}{0.556}{$-$0.071} & \rpxHCell{rpxHR}{0.620}{0.004} & \rpxHCell{rpxHR}{0.548}{0.392} & \rpxHCell{rpxHR}{0.416}{\underline{0.307}} & \rpxHCell{rpxHR}{0.464}{0.338} & \rpxHCell{rpxHR}{0.558}{0.398} \\
PaliGemma 2 3B & \rpxHCell{rpxHR}{0.462}{0.276} & \rpxHCell{rpxHR}{0.397}{\underline{0.230}} & \rpxHCell{rpxHR}{0.453}{0.270} & \rpxHCell{rpxHR}{0.626}{0.393} & \rpxHCell{rpxHR}{0.665}{0.057} & \rpxHCell{rpxHR}{0.584}{\underline{$-$0.038}} & \rpxHCell{rpxHR}{0.588}{$-$0.033} & \rpxHCell{rpxHR}{0.681}{0.076} & \rpxHCell{rpxHR}{0.442}{0.324} & \rpxHCell{rpxHR}{0.358}{\underline{0.270}} & \rpxHCell{rpxHR}{0.395}{0.294} & \rpxHCell{rpxHR}{0.583}{0.414} \\
DeepSeek-VL2 4.5B & \rpxHCell{rpxHR}{0.573}{0.355} & \rpxHCell{rpxHR}{0.386}{\underline{0.222}} & \rpxHCell{rpxHR}{0.489}{0.295} & \rpxHCell{rpxHR}{0.733}{0.469} & \rpxHCell{rpxHR}{0.803}{0.219} & \rpxHCell{rpxHR}{0.651}{\underline{0.041}} & \rpxHCell{rpxHR}{0.708}{0.108} & \rpxHCell{rpxHR}{0.807}{0.224} & \rpxHCell{rpxHR}{0.592}{0.420} & \rpxHCell{rpxHR}{0.369}{\underline{0.277}} & \rpxHCell{rpxHR}{0.477}{0.346} & \rpxHCell{rpxHR}{0.781}{0.541} \\
DeepSeek-VL2 1.0B & \rpxHCell{rpxHR}{0.201}{0.090} & \rpxHCell{rpxHR}{0.150}{\underline{0.054}} & \rpxHCell{rpxHR}{0.171}{0.069} & \rpxHCell{rpxHR}{0.233}{0.113} & \rpxHCell{rpxHR}{0.571}{$-$0.053} & \rpxHCell{rpxHR}{0.524}{$-$0.108} & \rpxHCell{rpxHR}{0.540}{$-$0.090} & \rpxHCell{rpxHR}{0.410}{\underline{$-$0.242}} & \rpxHCell{rpxHR}{0.270}{0.214} & \rpxHCell{rpxHR}{0.150}{\underline{0.137}} & \rpxHCell{rpxHR}{0.181}{0.157} & \rpxHCell{rpxHR}{0.245}{0.198} \\
Florence 2 0.77B & \rpxHCell{rpxHR}{0.268}{0.138} & \rpxHCell{rpxHR}{0.255}{0.129} & \rpxHCell{rpxHR}{0.269}{0.139} & \rpxHCell{rpxHR}{0.250}{\underline{0.125}} & \rpxHCell{rpxHR}{0.308}{$-$0.362} & \rpxHCell{rpxHR}{0.300}{$-$0.371} & \rpxHCell{rpxHR}{0.280}{$-$0.394} & \rpxHCell{rpxHR}{0.245}{\underline{$-$0.435}} & \rpxHCell{rpxHR}{0.198}{0.168} & \rpxHCell{rpxHR}{0.181}{0.157} & \rpxHCell{rpxHR}{0.194}{0.165} & \rpxHCell{rpxHR}{0.172}{\underline{0.151}} \\
Florence 2 0.23B & \rpxHCell{rpxHR}{0.258}{0.131} & \rpxHCell{rpxHR}{0.240}{\underline{0.118}} & \rpxHCell{rpxHR}{0.251}{0.126} & \rpxHCell{rpxHR}{0.243}{0.120} & \rpxHCell{rpxHR}{0.349}{$-$0.314} & \rpxHCell{rpxHR}{0.303}{$-$0.368} & \rpxHCell{rpxHR}{0.292}{$-$0.380} & \rpxHCell{rpxHR}{0.276}{\underline{$-$0.399}} & \rpxHCell{rpxHR}{0.200}{0.169} & \rpxHCell{rpxHR}{0.166}{\underline{0.147}} & \rpxHCell{rpxHR}{0.173}{0.152} & \rpxHCell{rpxHR}{0.166}{\underline{0.147}} \\
\rpxHMid
\textcolor{rpxHMute}{\textit{Times worst}} & \textcolor{rpxHMute}{0} & \textcolor{rpxHMute}{10} & \textcolor{rpxHMute}{1} & \textcolor{rpxHMute}{1} & \textcolor{rpxHMute}{0} & \textcolor{rpxHMute}{7} & \textcolor{rpxHMute}{2} & \textcolor{rpxHMute}{3} & \textcolor{rpxHMute}{0} & \textcolor{rpxHMute}{10} & \textcolor{rpxHMute}{1} & \textcolor{rpxHMute}{2} \\
\rpxHBottom
\end{rpxfit}
\end{table*}


==> generated/scene_objects_table.tex <==
\begin{table*}\newcommand{\tsN}[2]{\textbf{\textcolor{tier#1}{#2}}}%
\newcommand{\tsOut}{\raisebox{0.2pt}{\textcolor{rpxOutdoor}{\rule{3.8pt}{3.8pt}}}\hspace{2pt}}%
\newcommand{\tsIn}{{\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.35pt}\raisebox{0.2pt}{\fcolorbox{rpxIndoorInk}{rpxIndoor}{\rule{0pt}{3.1pt}\rule{3.1pt}{0pt}}}}\hspace{2pt}}%
\newcommand{\tsVR}{{\color{rpxHMute!40}\vrule width 0.4pt}}%
\caption{Objects in each MOS scene, listed by their SOS catalogue ID (Table~\ref{tab:sos-canonical}); the set is identical in all three exocentric phases. Scene numbers are coloured by difficulty tier (\textcolor{tierE}{Easy}, \textcolor{tierM}{Medium}, \textcolor{tierH}{Hard}); \tsIn{}\,indoor and \tsOut{}\,outdoor scenes are marked, following the capture sites of Fig.~\ref{fig:appendix-capture-sites} (40 outdoor, 60 indoor).}
\label{tab:appendix-scene-objects}
\rpxHeatStyle{5.9}{0pt}%
\renewcommand{\arraystretch}{1.12}%
\begin{rpxfit}{\textwidth}{6}{@{\hspace{2pt}}r@{\hspace{4pt}}l@{\hspace{\tabcolsep}}!{\tsVR}@{\hspace{\tabcolsep}}r@{\hspace{4pt}}l@{\hspace{\tabcolsep}}!{\tsVR}@{\hspace{\tabcolsep}}r@{\hspace{4pt}}l@{\hspace{\tabcolsep}}!{\tsVR}@{\hspace{\tabcolsep}}r@{\hspace{4pt}}l@{\hspace{2pt}}}
\rpxHTop
\multicolumn{1}{@{\hspace{2pt}}r@{\hspace{4pt}}}{\rule{0pt}{9pt}\rpxHHead{scene}} & \rpxHHead{objects (SOS ID)} & \rpxHHead{scene} & \rpxHHead{objects (SOS ID)} & \rpxHHead{scene} & \rpxHHead{objects (SOS ID)} & \rpxHHead{scene} & \rpxHHead{objects (SOS ID)} \\
\rpxHMid
\tsOut\tsN{H}{001} & 1, 2, 11, 20, 23, 27, 39 & \tsOut\tsN{E}{026} & 6, 21, 38, 43, 48, 49, 65 & \tsOut\tsN{E}{051} & 3, 20, 28, 33, 44, 45, 70 & \tsIn\tsN{M}{076} & 11, 14, 35, 41, 42, 60, 63 \\
\tsOut\tsN{H}{002} & 28, 37, 42, 46, 52, 56, 66 & \tsOut\tsN{H}{027} & 1, 10, 22, 41, 50, 60, 66 & \tsOut\tsN{M}{052} & 11, 29, 31, 39, 43, 52, 54 & \tsIn\tsN{M}{077} & 3, 15, 17, 22, 23, 30, 38 \\
\tsOut\tsN{H}{003} & 3, 9, 31, 49, 50, 51, 54 & \tsOut\tsN{M}{028} & 8, 23, 29, 33, 54, 58, 59 & \tsOut\tsN{E}{053} & 7, 30, 32, 34, 56, 62, 68 & \tsIn\tsN{M}{078} & 18, 26, 32, 43, 44, 47, 69 \\
\tsOut\tsN{E}{004} & 4, 14, 44, 55, 62, 65, 69 & \tsOut\tsN{E}{029} & 11, 24, 31, 34, 46, 51, 70 & \tsOut\tsN{E}{054} & 4, 37, 41, 47, 49, 58, 63 & \tsIn\tsN{M}{079} & 2, 10, 12, 27, 33, 56, 59 \\
\tsOut\tsN{H}{005} & 7, 13, 17, 19, 25, 60, 63 & \tsOut\tsN{E}{030} & 3, 37, 40, 57, 67, 68, 69 & \tsOut\tsN{E}{055} & 18, 35, 40, 48, 51, 55, 59 & \tsIn\tsN{H}{080} & 1, 25, 29, 39, 46, 61, 68 \\
\addlinespace[1.5pt]
\tsIn\tsN{M}{006} & 12, 15, 30, 32, 34, 38, 59 & \tsIn\tsN{E}{031} & 8, 29, 38, 56, 58, 61, 65 & \tsIn\tsN{M}{056} & 1, 12, 27, 36, 53, 67, 69 & \tsOut\tsN{H}{081} & 3, 17, 18, 24, 35, 36, 66 \\
\tsIn\tsN{M}{007} & 16, 22, 40, 43, 58, 64, 67 & \tsIn\tsN{E}{032} & 5, 20, 25, 26, 33, 45, 63 & \tsIn\tsN{E}{057} & 2, 6, 17, 24, 25, 46, 64 & \tsOut\tsN{H}{082} & 26, 29, 30, 42, 44, 51, 61 \\
\tsIn\tsN{E}{008} & 5, 8, 24, 35, 47, 48, 53 & \tsIn\tsN{H}{033} & 1, 13, 15, 40, 53, 54, 68 & \tsIn\tsN{M}{058} & 9, 15, 19, 21, 26, 38, 60 & \tsOut\tsN{H}{083} & 10, 16, 21, 37, 45, 46, 67 \\
\tsIn\tsN{M}{009} & 6, 21, 26, 33, 36, 57, 61 & \tsIn\tsN{E}{034} & 12, 16, 19, 41, 55, 60, 62 & \tsIn\tsN{E}{059} & 5, 10, 13, 14, 22, 61, 66 & \tsOut\tsN{M}{084} & 4, 6, 8, 50, 56, 64, 69 \\
\tsIn\tsN{H}{010} & 10, 18, 29, 41, 45, 68, 70 & \tsIn\tsN{E}{035} & 2, 49, 50, 57, 59, 64, 69 & \tsIn\tsN{E}{060} & 8, 16, 23, 42, 50, 57, 65 & \tsOut\tsN{H}{085} & 2, 20, 38, 40, 41, 49, 58 \\
\addlinespace[1.5pt]
\tsIn\tsN{E}{011} & 3, 4, 29, 30, 46, 54, 56 & \tsIn\tsN{M}{036} & 11, 18, 24, 35, 46, 51, 67 & \tsIn\tsN{H}{061} & 5, 6, 7, 15, 19, 21, 28 & \tsIn\tsN{M}{086} & 9, 22, 25, 43, 47, 55, 60 \\
\tsIn\tsN{E}{012} & 2, 14, 48, 53, 57, 65, 66 & \tsIn\tsN{E}{037} & 3, 7, 22, 30, 34, 36, 39 & \tsIn\tsN{H}{062} & 14, 25, 30, 39, 41, 43, 59 & \tsIn\tsN{H}{087} & 1, 23, 31, 39, 62, 63, 65 \\
\tsIn\tsN{E}{013} & 6, 19, 22, 31, 39, 59, 61 & \tsIn\tsN{E}{038} & 4, 27, 37, 43, 47, 66, 70 & \tsIn\tsN{H}{063} & 18, 29, 37, 47, 60, 66, 70 & \tsIn\tsN{H}{088} & 14, 27, 28, 32, 34, 57, 59 \\
\tsIn\tsN{M}{014} & 5, 24, 27, 38, 42, 64, 70 & \tsIn\tsN{H}{039} & 6, 14, 17, 21, 31, 44, 48 & \tsIn\tsN{M}{064} & 13, 26, 31, 32, 40, 51, 69 & \tsIn\tsN{M}{089} & 7, 11, 15, 33, 52, 68, 70 \\
\tsIn\tsN{E}{015} & 9, 17, 25, 32, 34, 58, 67 & \tsIn\tsN{H}{040} & 9, 10, 23, 28, 32, 42, 52 & \tsIn\tsN{M}{065} & 3, 22, 24, 34, 35, 48, 57 & \tsIn\tsN{M}{090} & 5, 12, 13, 19, 48, 53, 54 \\
\addlinespace[1.5pt]
\tsIn\tsN{H}{016} & 10, 15, 16, 45, 47, 49, 63 & \tsOut\tsN{H}{041} & 13, 14, 28, 37, 44, 60, 69 & \tsIn\tsN{E}{066} & 2, 27, 42, 45, 53, 55, 56 & \tsOut\tsN{M}{091} & 23, 24, 39, 47, 51, 57, 60 \\
\tsIn\tsN{M}{017} & 23, 35, 36, 40, 41, 44, 62 & \tsOut\tsN{H}{042} & 42, 46, 53, 55, 65, 66, 67 & \tsIn\tsN{H}{067} & 11, 16, 36, 46, 50, 52, 58 & \tsOut\tsN{E}{092} & 11, 22, 29, 30, 31, 37, 42 \\
\tsIn\tsN{H}{018} & 7, 11, 20, 28, 43, 52 & \tsOut\tsN{H}{043} & 4, 15, 25, 30, 45, 56, 57 & \tsIn\tsN{E}{068} & 9, 23, 33, 57, 61, 62, 67 & \tsOut\tsN{E}{093} & 2, 3, 26, 44, 50, 63, 68 \\
\tsIn\tsN{H}{019} & 8, 21, 37, 50, 55, 68, 69 & \tsOut\tsN{H}{044} & 3, 5, 10, 40, 49, 59, 64 & \tsIn\tsN{M}{069} & 10, 12, 17, 49, 54, 64, 65 & \tsOut\tsN{E}{094} & 5, 9, 33, 36, 46, 55, 67 \\
\tsIn\tsN{H}{020} & 1, 12, 13, 18, 26, 33, 60 & \tsOut\tsN{H}{045} & 21, 22, 23, 32, 38, 41, 58 & \tsIn\tsN{M}{070} & 4, 8, 20, 38, 44, 63, 68 & \tsOut\tsN{H}{095} & 7, 10, 45, 62, 64, 66, 69 \\
\addlinespace[1.5pt]
\tsIn\tsN{M}{021} & 5, 7, 13, 20, 27, 28, 63 & \tsOut\tsN{H}{046} & 1, 6, 19, 29, 36, 43, 50 & \tsIn\tsN{E}{071} & 4, 8, 28, 37, 45, 49, 62 & \tsOut\tsN{H}{096} & 8, 12, 21, 27, 35, 52, 53 \\
\tsIn\tsN{E}{022} & 14, 25, 32, 47, 52, 53, 56 & \tsOut\tsN{M}{047} & 8, 9, 12, 18, 47, 52, 61 & \tsIn\tsN{M}{072} & 5, 9, 20, 31, 50, 66, 70 & \tsOut\tsN{M}{097} & 1, 14, 17, 41, 48, 58, 61 \\
\tsIn\tsN{E}{023} & 4, 12, 17, 26, 39, 42, 44 & \tsOut\tsN{M}{048} & 7, 20, 24, 26, 31, 63, 68 & \tsIn\tsN{E}{073} & 13, 16, 34, 36, 40, 52, 65 & \tsOut\tsN{H}{098} & 15, 18, 25, 28, 32, 34, 59 \\
\tsIn\tsN{E}{024} & 2, 9, 15, 16, 18, 19, 61 & \tsOut\tsN{H}{049} & 11, 17, 33, 39, 48, 51, 62 & \tsIn\tsN{M}{074} & 7, 19, 21, 53, 54, 58, 67 & \tsOut\tsN{M}{099} & 13, 16, 19, 20, 38, 56, 65 \\
\tsIn\tsN{M}{025} & 30, 35, 36, 45, 55, 62, 64 & \tsOut\tsN{M}{050} & 2, 16, 27, 34, 35, 54, 70 & \tsIn\tsN{E}{075} & 6, 24, 48, 51, 55, 57, 64 & \tsOut\tsN{M}{100} & 4, 6, 11, 40, 43, 49, 54, 70 \\
\rpxHBottom
\end{rpxfit}
\end{table*}


==> generated/sos_catalogue.tex <==
\begin{table*}[p]
\centering
\caption{Canonical SOS questionnaire catalogue: every object with one lightly normalized canonical category, colour, material, and function response.}
\label{tab:sos-canonical}
\definecolor{tcGold}{HTML}{FBEFD5}\definecolor{tcGoldH}{HTML}{F6E2B4}%
\rpxHeatStyle{6.4}{0pt}%
\renewcommand{\arraystretch}{1.08}%
\newcommand{\tcI}[1]{\textcolor{rpxHMute}{#1}}%
\newcommand{\tcC}[1]{\textcolor{rpxHMute}{#1}}%
\newcommand{\tcH}[1]{{\fontfamily{IBMPlexMono-TLF}\selectfont #1}}%
\newcommand{\tcA}[1]{{\fontsize{6.4}{6.4}\selectfont\color{rpxOutdoor}#1}}%
\begin{rpxfit}{\textwidth}{8}{@{\hspace{2pt}}r@{\hspace{5pt}}>{\bfseries}l@{\hspace{\tabcolsep}}@{\hspace{\tabcolsep}}>{\rmfamily\fontsize{7.4}{8.4}\selectfont}l@{\hspace{\tabcolsep}}@{\hspace{\tabcolsep}}>{\columncolor{tcGold}[\tabcolsep][\tabcolsep]\rmfamily\fontsize{7.4}{8.4}\selectfont}l@{\hspace{\tabcolsep}}@{\hspace{\tabcolsep}}>{\columncolor{tcGold}[\tabcolsep][\tabcolsep]\rmfamily\fontsize{7.4}{8.4}\selectfont}l@{\hspace{\tabcolsep}}@{\hspace{\tabcolsep}}>{\columncolor{tcGold}[\tabcolsep][\tabcolsep]\rmfamily\fontsize{7.4}{8.4}\selectfont}l@{\hspace{2pt}}}
\rpxHTop
\multicolumn{1}{@{\hspace{2pt}}r@{\hspace{5pt}}}{\rule{0pt}{9.4pt}\rpxHHead{ID}} & \tcH{\mdseries\rpxHHead{object}} & \tcH{\rpxHHead{category}} & \cellcolor{tcGoldH}\tcH{\tcA{colour}} & \cellcolor{tcGoldH}\tcH{\tcA{material}} & \cellcolor{tcGoldH}\tcH{\tcA{function}} \\
\rpxHMid
\tcI{1} & air duster can & \tcC{utilities} & grey & plastic/metal & cleaning \\
\tcI{2} & alarm clock & \tcC{clocks and watches} & silver & metal & waking up \\
\tcI{3} & apple & \tcC{food} & red & plant & eating \\
\tcI{4} & baking tray & \tcC{baking} & black & metal & baking food \\
\tcI{5} & banana & \tcC{fruit} & yellow & plastic & eating \\
\addlinespace[1.5pt]
\tcI{6} & baseball ball & \tcC{sports} & white & rubber & playing \\
\tcI{7} & basting brush & \tcC{office tools} & brown and blue & plastic & clean keyboard \\
\tcI{8} & beanie & \tcC{clothing} & purple blue and dark purple & fabric & fashion \\
\tcI{9} & bear & \tcC{toy} & grey & cotton & playing \\
\tcI{10} & book & \tcC{stationery} & white & paper & study \\
\addlinespace[1.5pt]
\tcI{11} & boot & \tcC{apparel} & white & leather & footwear \\
\tcI{12} & bowl & \tcC{utensil} & red & glass & keeps food inside it \\
\tcI{13} & cable & \tcC{accessories} & white & rubber & connect \\
\tcI{14} & candy bar & \tcC{food} & brown & plastic & eat \\
\tcI{15} & cleaning brush & \tcC{hygiene equipment} & white & plastic & cleaning \\
\addlinespace[1.5pt]
\tcI{16} & coffee bottle & \tcC{bottle} & brown & plastic & drinking \\
\tcI{17} & coffee can & \tcC{can} & red & metal & to eat \\
\tcI{18} & cracker box & \tcC{box} & red & plastic & eating \\
\tcI{19} & cup & \tcC{food tool} & yellow and white & paper & drinking liquids \\
\tcI{20} & doll & \tcC{toys} & red & rubber & playing \\
\addlinespace[1.5pt]
\tcI{21} & fry pan & \tcC{kitchenware} & black & cast iron & cooking \\
\tcI{22} & food bag & \tcC{food} & yellow green & plastic & eating \\
\tcI{23} & game controller & \tcC{gaming} & black & plastic & gaming \\
\tcI{24} & glove & \tcC{clothing accessory} & black & cloth & going outside in the cold \\
\tcI{25} & glue bottle & \tcC{holding} & white orange and black & plastic & glue things \\
\addlinespace[1.5pt]
\tcI{26} & hair brush & \tcC{beauty} & black & plastic & styling \\
\tcI{27} & hammer & \tcC{tool} & black & metal & hammering \\
\tcI{28} & handy pot & \tcC{utensil} & black & metal \& plastic & cooking \\
\tcI{29} & hat & \tcC{accessory} & white & cotton & for head \\
\tcI{30} & headphone & \tcC{technology} & black & plastic & listening \\
\addlinespace[1.5pt]
\tcI{31} & helmet & \tcC{safety} & purple & fiberglass & wearable \\
\tcI{32} & instant noodle packet & \tcC{packet} & red & noodles & eating \\
\tcI{33} & jar & \tcC{storage} & yellow & glass & storing food \\
\tcI{34} & jello box & \tcC{box} & white & paper & eating \\
\tcI{35} & juice pouch & \tcC{container} & orange & plastic & drink \\
\addlinespace[1.5pt]
\tcI{36} & kettle & \tcC{utensil} & silver & plastic and metal & tea or water \\
\tcI{37} & knife & \tcC{kitchen accessories} & red and silver & steel & cut food \\
\tcI{38} & ladle & \tcC{utensils} & green & plastic & eating \\
\tcI{39} & lion & \tcC{toys} & tan & plastic & play \\
\tcI{40} & marker & \tcC{office tools} & black and yellow & plastic & writing \\
\addlinespace[1.5pt]
\tcI{41} & meat can & \tcC{can} & blue & metal & eating \\
\tcI{42} & milk box & \tcC{food} & red & paper & eating \\
\tcI{43} & milk jug & \tcC{container} & white & plastic & containing liquid \\
\tcI{44} & mouse & \tcC{computer accessories} & blue & plastic & working \\
\tcI{45} & mug & \tcC{kitchen accessory} & blue & porcelain & drink tea \\
\addlinespace[1.5pt]
\tcI{46} & mustard bottle & \tcC{food} & yellow and white & plastic & seasoning \\
\tcI{47} & pear & \tcC{fruit} & green & plastic & eating \\
\tcI{48} & peeler & \tcC{kitchen tool} & black & plastic & peeling the fruits and vegetables \\
\tcI{49} & power drill & \tcC{tool} & black & metal & drilling \\
\tcI{50} & pringles can & \tcC{food} & green & paper & eating \\
\addlinespace[1.5pt]
\tcI{51} & pump bottle & \tcC{beauty product} & white & plastic & lotion \\
\tcI{52} & remote controller & \tcC{tool} & black & plastic & change channel \\
\tcI{53} & root beer bottle & \tcC{drink} & brown & plastic & drinking \\
\tcI{54} & scissors & \tcC{tool} & grey & steel & cutting \\
\tcI{55} & shampoo bottle & \tcC{beauty} & white & plastic & scrubbing \\
\addlinespace[1.5pt]
\tcI{56} & shoe & \tcC{apparel} & white green and blue & rubber & running \\
\tcI{57} & soda can & \tcC{food} & blue & metal & drink \\
\tcI{58} & soft scrub cleanser bottle & \tcC{bottle} & white & plastic & cleaning \\
\tcI{59} & soup can & \tcC{food} & red & metal & drink \\
\tcI{60} & spatula & \tcC{utensil} & brown & wood & cooking \\
\addlinespace[1.5pt]
\tcI{61} & sponge & \tcC{cleaning tool} & blue & glycerin & cleaning \\
\tcI{62} & spray bottle & \tcC{tools} & blue & plastic & spray \\
\tcI{63} & t-handle & \tcC{tool} & black & metal & remove something \\
\tcI{64} & tape measure & \tcC{tool} & black & metal & to measure \\
\tcI{65} & teapot & \tcC{utensils} & white & plastic & store \\
\addlinespace[1.5pt]
\tcI{66} & tong & \tcC{utensils} & silver & metal & eating \\
\tcI{67} & toothpaste & \tcC{health} & blue & plastic & brushing tooth \\
\tcI{68} & towel & \tcC{cleaning tool} & yellow & cloth & clean \\
\tcI{69} & umbrella & \tcC{accessory} & brown & plastic & covers and protect from rain \\
\tcI{70} & water bottle & \tcC{bottle} & green & plastic & storing liquids \\
\rpxHBottom
\end{rpxfit}
\end{table*}

